The Importance of Prompt Tuning for Automated Neuron Explanations

Recent advances have greatly increased the capabilities of large language models (LLMs), but our understanding of the models and their safety has not progressed as fast. In this paper we aim to understand LLMs deeper by studying their individual neurons. We build upon previous work showing large language models such as GPT-4 can be useful in explaining what each neuron in a language model does. Specifically, we analyze the effect of the prompt used to generate explanations and show that reformatting the explanation prompt in a more natural way can significantly improve neuron explanation quality and greatly reduce computational cost. We demonstrate the effects of our new prompts in three different ways, incorporating both automated and human evaluations.

==> Table/model_details.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll} 
\toprule
& & & Per 1k token &Cost per1k token \\ 
Model:& Release Date:& Model size:& cost (input): & cost (output):\\ \midrule
GPT-4& March 2023& $1.8\times 10^{12}$ parameters, 120 layers&  \$0.03&\$0.06\\
GPT-3.5-Turbo& March 2022& $1.8\times 10^{12}$ 3.75 billion parameters across 96 layers&  \$0.0015&\$0.002\\
GPT-3.5-Turbo-Instruct& September 2023& 375 billion parameters across 96 layers&  \$0.0015&\$0.002\\
\bottomrule
\end{tabular}
}
\vspace{1em}
\caption{General model information}
\label{tab:model_size}
\end{table}


==> for_later.tex <==
%auto-ignore

%Additional background

%\textbf{Neuron-level Interpretation of LLMs.}
%\cite{sajjad2022neuronlevel} provides a good overview, dividing existing methods  into five categories: visualization, corpus-based methods, probing-based methods, causation-based methods, and miscellaneous methods. 
%Visualization methods visualize the activations of a neuron and manually identify the underlying concept over a set of sentences \citep{karpathy2015visualizing, fyshe2015compositional}. 
%Corpus-based methods discover the role of neurons by aggregating statistics of neuron activations over large datasets \citep{kadar2017representation, na2019discovery, mu2020compositional}. Probing-based methods train diagnostic classifiers (either a linear classifer \citep{dalvi2019one} or a Gaussian classifier \citep{hennigen2020intrinsic}) over activations to identify neurons with respect to pre-defined concepts. 
%Causation-based methods identify neurons with respect to the model’s prediction either through ablation \citep{lakretz2019emergence}, where they notice the effect of a neuron on the model’s performance by varying its value, or knowledge attribution methods \citep{dai2021knowledge}, where they highlight the importance of input features and neurons with respect to a prediction. We refer readers to \cite{sajjad2022neuronlevel} for a more comprehensive review of neuron-level interpretability of deep NLP models. 
% Miscellaneous methods are a diverse set of methods that do not fit into the above defined categories, including corpus generation \citep{poerner2018interpretable}, matrix factorization \citep{alammar2020interfaces}, clustering \citep{dalvi2020analyzing}, and multi model search \citep{bau2018identifying}.
%Our method in this paper and~\cite{bills2023language} can be viewed as a corpus based method.

% % comment the simulation part out for now
% Finally, they propose a new way to evaluate the quality of these descriptions called simulation, in which the generated explanation is scored against the true activations. By feeding the generated explanation and a new text into another LLM known as the \textit{simulator model} (also GPT-4 in their case), the simulator model can predict the activations of a neuron based on the provided description. The simulated and true activations can then be compared, resulting in a score for the generated explanation. A higher score equates to an explanation that more accurately describes the activations. 

% They also propose a few additions to this approach, such as revising the predictions and looking into interpretable directions. The neuron activations they recorded and explanations generated using their full pipeline are publicly available, which we will later utilize for our own testing.. 

%They can generate a summary about the activations of each neuron by feeding the activations of a neuron into an LLM. The LLMs used in this paper refer to OpenAI's GPT models. 

%When a user enters a prompt into GPT, the prompt is in the form of english plaintext. A neural network such as GPT requires the input to be in numerical form. Therefore, text embedding, an algorithm that turns text into a numerical vector, is required. Many text-embedding have been created in the past, with the simplest being the bag of words method. Each word is assigned an index in an N-dimensional vector, and the index is incremented by one each time the word appears in the text. GPT uses its own text-embedding model that was trained along with GPT itself. 

%When looking at specific neurons in a GPT model, known as the subject model or the model being analyzed, the parts of the word vector that reached a neuron can be calculated. Since each part of a word vector is associated with certain text from the original plaintext, we can find the exact parts of words, known as tokens, that reached a specific neuron. Depending on how significantly the text that reaches the neuron triggers the activation function, the text can be given a value of how activating it is to the neuron. 

%With a set of activating texts, an explanation can be generated that summarizes the words in a simple phrase. This explanation is generated by a GPT model, referred to as the generator model. 


% \subsection{GPT models}
% \lily{\todo{TODO for Kengchi+Yilan:} introduce the architecture of GPT models, this will help the reader to know what we are interpreting (you can check out the text we currently have in sec 3.1). Also give a brief overview on different GPT models' difference.}
% \kengchi{Added two paragraphs.}


%In this paper, we focus on the neurons in the MLP layers. In particular, we use the same subject model GPT-2 (XL) as \citep{bills2023language}, which is the last open-sourced GPT model by OpenAI with 48 MLP layers and 6400 neurons per layer, resulting in a total of 307,200 unique MLP neurons. For the explainer model in Fig~\ref{fig:overview}, we use GPT-3.5-Turbo, GPT-4 models, and for the simulator model in section 3.4, we use the very recently released GPT-3.5-Turbo-Instruct. See Table \ref{tab:model_size} for more details on the models. 
%\tuomas{removed this since its also discussed in section 4.}

%\tuomas{Do we need this paragraph?}As the first model of its kind, GPT-1 \cite{radford2018improving} proposed learning a generative model by unsupervised pre-training followed by supervised fine-tuning for NLP tasks. 
%GPT-1 was trained on Book Corpus and had around 170 million parameters.
%GPT-2 \cite{radford2019language} added more parameters to the model (1.5 billion for the largest model), trained on larger dataset (40GB WebText data) and introduced the concept of task conditioning---for different tasks, the model is expected to produce different outputs for the same inputs.
%GPT-3 \cite{brown2020language} was trained on a mix of five different corpora and had 175 billion parameters.
%It introduced the concept of in-context learning---one or a few examples are given to the model to provide context, showing boost of performance.

%We also explored different methods measuring sentence similarity, but found the sentence similarity for AdaV2 to perform the best. In addition, different methods mostly agreed on which prompting method performed the best. More details can be found in the Appendix \ref{sec:apdx_gpt_comparison} and \ref{sec:apdx_gpt_comparison2}. \tuomas{These Appendix sections need to be made a lot nicer if we want to include this.}

\subsection{Method 2: GPT Comparison} 
\label{sec:apdx_gpt_comparison}
Another potential method for comparing similarity between explanations is through an evaluator model. We used GPT-3.5 as the evaluator. The base plan is to give GPT two explanations and ask for a similarity ranking from 1-10. When testing GPT Comparison Models, we ran the comparison on 5k pairs of explanations, taken from the top 1k neurons with explanations generated from the 5 prompting methods.

Some issues that came up were consistency and accuracy. When given the same pair of sentences twice, GPT-3.5 oftentimes gave different rankings each time. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/GPT_inaccuracy.png}
    \caption{\lily{what's this fig? \todo{@Justin+Arjun:} make this figure nicer and clearer. It's unclear what it is by looking at it.} [Justin: This figure is going to be irrelevant once we delete V1-V6 content as per Tuomas's advice, skipping]}
    \label{fig:enter-label}
\end{figure}
We attempted to solve the issues through few-shot prompting. This method requires sending the evaluator model various examples of the problem being asked. In our case, by sending example pairs of explanations and their similarity ranking, GPT has a baseline to calculate its similarity ranking off of. 

Example of a few-shot prompt sent to GPT: \lily{reformat it nicer}
\begin{itemize}
    \item[] Here are some example pairs of explanations and their ranks. You will receive 2 explanations, then the ranking value of    their similarity.\newline
    first explanation: words related to crisis situations and their resolution\newline
    second explanation: words related to medical and humanitarian crises\newline
    8
\end{itemize}

GPT Comparison Methods V1, V2, and V3 tested different combinations of few-shot prompts. While both accuracy and consistency improved, some inaccurate rankings remained. The following examples illustrating these inaccuracies list the ground truth explanation, then the generated explanation, and lastly the similarity ranking. \lily{reformat it nicer}
\begin{itemize}
    \item[] instances of the word 'attempt'\newline
    words related to trying or making an effort\newline
    7.5\newline
    instances of the word 'attempt'\newline
    words related to trying or striving to achieve something\newline
    9.5
\end{itemize}

To combat the persisting errors, V4 and V5 were created from different approaches. V4 started with an empty few-shot prompt list. When GPT made an evaluation, the explanation pair along with the ranking that GPT just generated were added to the few-shot prompt. Then, in the next cycle, the updated few-shot prompt was sent to GPT. This way, GPT could base its rankings off of its previous ranking moments ago. 

V5 sent 5 explanation pairs to GPT at once, one explanation pair for each prompting method. GPT could compare the pairs with each other to come up with a better ranking relative to each other. 

V6 implemented chain-of-thought, a slightly altered variant of few-shot prompts. Instead of sending explanation pairs and their corresponding ranking, GPT would receive the explanation pair, ranking, and the explanation why the ranking was given. 

\lily{\todo{TODO for Arjun+Justin:} Illustrate V1-V6 in a figure}

[Justin: This might be irrelevant once we delete V1-V6 content as per Tuomas's advice, but could be helpful to just have a single figure summarizing V1-V6, discuss in zoom?]

\subsection{Experiment 2: Evaluating quality of surrogate methods}
\label{sec:apdx_gpt_comparison2}
GPT Comparison V4, V5, and V6 were compared with each other along with AdaCS. First, we define a function that returns the minimum ranking subtracted from the maximum ranking, known as the range.

The function is given groups of 5 rankings, one for each prompting method explaining the same neuron. If this range is larger than a set variable, such as 3, then add the tested neuron to a list of controversial neurons. These neurons' corresponding explanations generated by each prompting method, which are shown to be up for debate by the varying rankings, can be ranked by the top 4 comparison methods. Finally, we can compare the rankings of the comparison methods to our manual ranking. 

When looking at the accuracy of each comparison method, we focus on the relative rankings of explanations or the ordering based on rankings. Many of these models are powered by relative analysis. In other words, rankings for new explanations are created off of rankings for past explanations. If a ranking seems off on its own but makes sense when looking at its placement relative to the rankings of other explanations, the ranking is considered accurate. 

Here is example analysis regarding a single neuron: \lily{reformat it nicer}
\begin{itemize}
\item[] Neuron Viewer:  words related to time, specifically morning events.\newline
HS: words related to time of day, specifically morning, and action-related terms like flash and rush.\newline
H: phrases related to time, specifically indicating moments or periods of the day.\newline
S: words and phrases related to time, specifically morning or early events or activities that occur during the morning.\newline
O: news or current event topics related to politics or government actions.\newline
AVHS: words related to time of day, particularly "morning", as well as words related to information dissemination or urgency, such as "flash" and "rush".\newline
V4 ranking: ['S: 9.5', 'H: 8.5', 'AVHS: 8.5', 'HS: 7.5', 'O: 2.5']\newline
V5 ranking: ['S: 10.0', 'AVHS: 9.0', 'HS: 8.0', 'H: 6.0', 'O: 0.0']\newline
COTv1 ranking: ['S: 8.5', 'HS: 7.5', 'H: 7.5', 'O: 7.5', 'AVHS: 7.5']\newline
AdaCS ranking: ['S: 0.948', 'HS: 0.903', 'AVHS: 0.893', 'H: 0.888', 'O: 0.789']\newline \newline
Our manual ordering (from best to worst): S, HS, AVHS, H, O\newline
Best comparison model based on similarity to our manual ranking(from best to worst): AdaCS, V5, V4, COTv1

\end{itemize}

AdaCS is consistently the best model when the rankings of explanations or rankings of models are not up for debate. AdaCS seems to give rankings that range in the upper bound of [0,1] even when a certain explanation is very inaccurate. This analysis shows why directly comparing rankings for individual explanations may not include the full picture. It may seem as if AdaCS is always giving high rankings to every explanation when in reality the relative rankings are clearly different.


\section{Save for blog post}

    Recently, ChatGPT has seen a rapid explosion in popularity due to its abilities such as coding assistance code or answering questions across a huge range of topics. However, even before Large Language Models (LLM) like ChatGPT took the spotlight, LLMs had already started playing a major role in technology. For example Google has utilized BERT \todo{CITE} based models for handling a lot of their search traffic, and many chatbots or translation methods rely on language models. 


        \tuomas{Reduced historical narrative here, focused more on what they're currently able to do.}
    
    %In 2019, Google announced their new language model, BERT. Pre-trained on Wikipedia data, BERT helps computers understand the subtle similarities and differences in text. BERT would eventually handle a majority of English queries in the Google search engine.
    
    %Apart from BERT, primitive versions of GPT were already in the works. Models such as GPT-2 and GPT-3 steadily improved without catching much public attention. When OpenAI released ChatGPT, casual users could use the ChatGPT interface to directly query the GPT model without having to go through any programming. The power of LLMs were suddenly visible to the public, and the use of ChatGPT in daily life only grew from there. 
 
    But how does the neural network behind the GPT model that powers ChatGPT work? The "thoughts" of GPT lay shrouded in fog. To humans, the numbers that determine the structure of a neural network are meaningless in its raw form. If these numbers planted bias within GPT's judgment, humans would be none the wiser. This obscurity becomes a problem when systems like ChatGPT are widely used in all sectors of work.
    A deeper understanding of GPT is important when probing for flaws, maintaining security, and keeping consistency. This is needed to ensure models can for example refrain from lying or don't in harmful pursuits such as providing advice on how to build weapons.
    
    %With GPT-4's release, a model displaying significantly improved control over language and knowledge, the interpretability of LLMs has only grown into a more pressing matter. 

    
    In this paper, we improve on existing methods to describe individual neurons inside LLMs. Specifically, we show that different, more natural prompts can improve the quality of single neuron explanations proposed by  \cite{bills2023language}. We experiment we several different prompting methods, and show that simpler, more natural examples can greatly improve quality of neuron explanations in both automated and human evaluations.


% \subsection{Neural Networks}
% A neural network can be thought of as a pipeline, passing from layer to layer. Each layer contains neurons and the neurons of each layer are all connected to each of the neurons of the next layer. A neuron has a specific weight value and bias value that alters the output of the neuron. When a neuron receives input from neurons from the previous layer, it calculates the output using its inputs, weights and biases. The output is sent to an activation function, which determines whether or not the output is significant enough to be sent to the next layer. If the activation function determines that the output is very significant, the input that was sent into this neuron is considered highly activating for this specific neuron. Every neuron will have a different group of activating inputs. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Images/NN_image1.png}
%     \caption{A Simple Neural Network Diagram}
%     \label{fig:1}
% \end{figure}
